CG-OoO: Energy-Efficient Coarse-Grain Out-of-Order Execution

We introduce the Coarse-Grain Out-of-Order (CG- OoO) general purpose processor designed to achieve close to In-Order processor energy while maintaining Out-of-Order (OoO) performance. CG-OoO is an energy-performance proportional general purpose architecture that scales according to the program load. Block-level code processing is at the heart of the this architecture; CG-OoO speculates, fetches, schedules, and commits code at block-level granularity. It eliminates unnecessary accesses to energy consuming tables, and turns large tables into smaller and distributed tables that are cheaper to access. CG-OoO leverages compiler-level code optimizations to deliver efficient static code, and exploits dynamic instruction-level parallelism and block-level parallelism. CG-OoO introduces Skipahead issue, a complexity effective, limited out-of-order instruction scheduling model. Through the energy efficiency techniques applied to the compiler and processor pipeline stages, CG-OoO closes 64% of the average energy gap between the In-Order and Out-of-Order baseline processors at the performance of the OoO baseline. This makes CG-OoO 1.9x more efficient than the OoO on the energy-delay product inverse metric.

==> acknowledgements.tex <==
\section{Acknowledgements\label{sec:ack}}
TODO


==> discussion.tex <==
\section{Discussion}\label{sec:discussion}



==> revision.tex <==
\newcommand{\Revision}{ba74616}

